GeoPix: Multi-Modal Large Language Model for Pixel-level Image Understanding in Remote Sensing

Multi-modal large language models (MLLMs) have achieved remarkable success in image- and region-level remote sensing (RS) image understanding tasks, such as image captioning, visual question answering, and visual grounding. However, existing RS MLLMs lack the pixel-level dialogue capability, which involves responding to user instructions with segmentation masks for specific instances. In this paper, we propose GeoPix, a RS MLLM that extends image understanding capabilities to the pixel level. This is achieved by equipping the MLLM with a mask predictor, which transforms visual features from the vision encoder into masks conditioned on the LLM's segmentation token embeddings. To facilitate the segmentation of multi-scale objects in RS imagery, a class-wise learnable memory module is integrated into the mask predictor to capture and store class-wise geo-context at the instance level across the entire dataset. In addition, to address the absence of large-scale datasets for training pixel-level RS MLLMs, we construct the GeoPixInstruct dataset, comprising 65,463 images and 140,412 instances, with each instance annotated with text descriptions, bounding boxes, and masks. Furthermore, we develop a two-stage training strategy to balance the distinct requirements of text generation and masks prediction in multi-modal multi-task optimization. Extensive experiments verify the effectiveness and superiority of GeoPix in pixel-level segmentation tasks, while also maintaining competitive performance in image- and region-level benchmarks.

==> resp_tabs/alb_design_memory.tex <==
\begin{table}[h]
\centering
\caption{Comparison of memory capacity and memory fusion. The upper part of the table compares different memory capacities. The lower part evaluates the performance of various memory fusion methods under a fixed capacity.}
\label{table:resp_memory_design}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{Design of CLM module} & \multirow{2}{*}{Learnable Parameter}  & \multicolumn{2}{c|}{SIOR-T} \\ \cline{3-4} 
    &    & mIoU       & cIoU      \\ \hline
\multicolumn{4}{|c|}{\textit{Memory Capacity \( N\) (Fusion by Conv3D)}} \\ \hline
\rz{w/o CLM module}    &  0  & 76.56      & 83.25     \\
32     &  2.7K  & 80.77      & 88.12     \\
64     &  2.7K  & \textbf{84.25}  & 89.82     \\
256    &  2.7K  & 83.88      & \textbf{89.99}      \\ \hline
\multicolumn{4}{|c|}{\textit{Memory Fusion (Capacity = 64)}} \\ \hline
Argmax   &  0  &  79.24  & 87.21     \\
Conv2D   &  2.7K    &  83.88  & 89.42     \\
Conv3D   &  2.7K    &  \textbf{84.25}  & 89.82      \\ 
Attention       &  532.8K  &  83.91  & 88.92     \\
Dual Attention       &  34.6M   &  84.20  & \textbf{89.95}      \\ \hline
\end{tabular}
}
\end{table}

==> resp_tabs/data.tex <==
\begin{table}[!ht]
\centering
\caption{Statistics of GeoPixInstruct. The size refers to the width and height of square images. \rz{The GSD refers to the ground sampling distance measured in meters.} \(\varphi\) represents the number of instances per image and the \(\theta\) represents the mask coverage ratio within the images.}
\label{table:resp_data}
% \resizebox{0.5\linewidth}{!}{%
\begin{tabular}{lccccccc}
\hline
Subset & \#Img. & \#Cat. & \#Inst. & Size  & \rz{GSD (m)} & Avg. \(\varphi\)   & Avg. \(\theta\)           \\ \hline
SIOR-T & 17,402 & 20     & 38,320  & 800   & \rz{0.5-30}  & 2.20              & 4.34                 \\
FAST-T & 38,565 & 37     & 77,276  & 600   & \rz{0.3-0.8} & 2.61              & 1.12                 \\
SOTA-T & 9,038  & 18     & 24,816  & 1024  & \rz{0.1-4.5} & 2.00              & 0.94                 \\ \hline
\end{tabular}
% }
\end{table}

==> resp_tabs/seg.tex <==
\begin{table}[h]
\centering
\caption{Comparison of model performance on the multi-referring segmentation in the GeoPixInstruct. \rz{VG refers to Visual Grounding, with the corresponding IoU calculated for the bounding boxes. VG+SAM/SAM2 refers to using the Visual Grounding results as conditions for prediction with SAM/SAM2. $^\dagger$ indicates that the models are trained using the proposed two-stage training strategy. $^*$ indicates that the models are specialized in referring segmentation.}}
\label{table:resp_seg}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline
\multirow{3}{*}{Method}  & \multicolumn{5}{c|}{SIOR-T}                           & \multicolumn{5}{c|}{FAST-T}                           & \multicolumn{5}{c}{SOTA-T}                           \\ \cline{2-16} 
                                          &   \rz{\rz{Small}} & \rz{\rz{Medium}} & \rz{\rz{Large}} & \multicolumn{2}{c|}{Overall} & \rz{Small} & \rz{Medium} & \rz{Large} & \multicolumn{2}{c|}{Overall} & \rz{Small} & \rz{Medium} & \rz{Large} & \multicolumn{2}{c}{Overall} \\
                                           & \rz{mIoU}  & \rz{mIoU}   & \rz{mIoU}  & mIoU          & cIoU         & \rz{mIoU}  & \rz{mIoU}   & \rz{mIoU}  & mIoU          & cIoU         & \rz{mIoU}  & \rz{mIoU}   & \rz{mIoU}  & mIoU         & cIoU         \\ \hline
RRSIS$^*$ & \rz{36.98} & \rz{73.57}  & \rz{78.99} & 57.80         & 72.85        & \rz{51.75} & \rz{\textbf{72.63}}  & \rz{77.25} & 49.46         & 57.14        & \rz{21.27} & \rz{51.97}  & \rz{\textbf{75.73}} & 24.30        & 42.89        \\
RMSIN$^*$ & \rz{60.72} & \rz{79.40}  & \rz{86.24} & 65.10         & 78.27        & \rz{\textbf{55.48}} & \rz{65.82}  & \rz{64.90} & \textbf{56.59}         & 56.88        & \rz{\textbf{42.60}} & \rz{55.25}  & \rz{53.42} & \textbf{44.42}        & 45.12        \\ \hline
LISA  & \rz{55.11} & \rz{80.73}  & \rz{85.38} & 69.48         & 79.61        & \rz{38.73} & \rz{48.10}  & \rz{63.68} & 40.14         & 40.81        & \rz{30.63} & \rz{44.40}  & \rz{66.50} & 32.29        & 37.69        \\
PixelLM & \rz{45.03} & \rz{72.27}  & \rz{77.47} & 60.37         & 72.73        & \rz{34.21} & \rz{47.70}  & \rz{49.16} & 36.05         & 40.61        & \rz{23.42} & \rz{38.37}  & \rz{52.19} & 25.39        & 35.48        \\ \hline
\rz{LISA$^\dagger$}                                & \rz{62.48} & \rz{86.37}  & \rz{95.75} & \rz{82.14}         & \rz{87.38}        & \rz{38.62} & \rz{49.42}  & \rz{75.82} & \rz{41.98}         & \rz{52.05}        & \rz{27.88} & \rz{46.86}  & \rz{68.23} & \rz{31.02}        & \rz{41.88}        \\
\rz{PixelLM$^\dagger$}                          & \rz{66.93} & \rz{85.71}  & \rz{93.28} & \rz{78.05}         & \rz{86.97}        & \rz{40.23} & \rz{52.25}  & \rz{77.28} & \rz{42.34}         & \rz{52.17}        & \rz{29.26} & \rz{47.42}  & \rz{55.83} & \rz{30.12}        & \rz{41.22}        \\ \hline
\rz{VG}        & \rz{33.56} & \rz{66.30}  & \rz{71.96} & \rz{51.40}         & \rz{63.15}        & \rz{30.42} & \rz{52.69}  & \rz{62.95} & \rz{33.08}         & \rz{43.05}        & \rz{22.70} & \rz{56.47}  & \rz{75.19} & \rz{26.35}        & \rz{46.72}        \\ 
\rz{VG+SAM}                 & \rz{40.37} & \rz{79.21}  & \rz{74.38} & \rz{60.58}         & \rz{69.58}        & \rz{37.22} & \rz{57.70}  & \rz{40.15} & \rz{39.36}         & \rz{37.98}        & \rz{25.83} & \rz{57.87}  & \rz{43.70} & \rz{29.36}        & \rz{39.07}        \\
\rz{VG+SAM2}              & \rz{34.30} & \rz{73.36}  & \rz{62.62} & \rz{54.15}         & \rz{62.10}        & \rz{31.69} & \rz{55.04}  & \rz{47.91} & \rz{34.27}         & \rz{37.14}        & \rz{21.11} & \rz{53.18}  & \rz{38.60} & \rz{24.40}        & \rz{33.27}      \\ 

\textbf{GeoPix} & \rz{\textbf{75.49}} & \rz{\textbf{92.37}}  & \rz{\textbf{96.27}} & \textbf{84.25}         & \textbf{89.82}        & \rz{50.73} & \rz{71.76}  & \rz{\textbf{80.63}} & 53.54         & \textbf{57.25}        & \rz{32.43} & \rz{\textbf{58.01}}  & \rz{59.88} & 35.37        & \textbf{45.24}        \\ \hline
\end{tabular}
}
\end{table}

==> resp_tabs/seg_1.tex <==
\begin{table}[h]
\centering
\caption{Comparison of model performance on the multi-referring segmentation in the GeoPixInstruct. \rz{VG refers to Visual Grounding, with the corresponding IoU calculated for the bounding boxes. VG+SAM/SAM2 refers to using the Visual Grounding results as conditions for prediction with SAM/SAM2. $^\dagger$ indicates that the models are trained using the proposed two-stage training strategy. $^*$ indicates that the models are specialized in referring segmentation.}}
\label{table:resp_seg1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline
\multirow{3}{*}{Method}  & \multicolumn{5}{c|}{SIOR-T}                           & \multicolumn{5}{c|}{FAST-T}                           & \multicolumn{5}{c}{SOTA-T}                           \\ \cline{2-16} 
                                          &   \rz{\rz{Small}} & \rz{\rz{Medium}} & \rz{\rz{Large}} & \multicolumn{2}{c|}{Overall} & \rz{Small} & \rz{Medium} & \rz{Large} & \multicolumn{2}{c|}{Overall} & \rz{Small} & \rz{Medium} & \rz{Large} & \multicolumn{2}{c}{Overall} \\
                                           & \rz{mIoU}  & \rz{mIoU}   & \rz{mIoU}  & mIoU          & cIoU         & \rz{mIoU}  & \rz{mIoU}   & \rz{mIoU}  & mIoU          & cIoU         & \rz{mIoU}  & \rz{mIoU}   & \rz{mIoU}  & mIoU         & cIoU         \\ \hline
RRSIS$^*$ & \rz{36.98} & \rz{73.57}  & \rz{78.99} & 57.80         & 72.85        & \rz{51.75} & \rz{\textbf{72.63}}  & \rz{77.25} & 49.46         & 57.14        & \rz{21.27} & \rz{51.97}  & \rz{\textbf{75.73}} & 24.30        & 42.89        \\
RMSIN$^*$ & \rz{60.72} & \rz{79.40}  & \rz{86.24} & 65.10         & 78.27        & \rz{\textbf{55.48}} & \rz{65.82}  & \rz{64.90} & \textbf{56.59}         & 56.88        & \rz{\textbf{42.60}} & \rz{55.25}  & \rz{53.42} & \textbf{44.42}        & 45.12        \\ \hline
LISA  & \rz{55.11} & \rz{80.73}  & \rz{85.38} & 69.48         & 79.61        & \rz{38.73} & \rz{48.10}  & \rz{63.68} & 40.14         & 40.81        & \rz{30.63} & \rz{44.40}  & \rz{66.50} & 32.29        & 37.69        \\
PixelLM & \rz{45.03} & \rz{72.27}  & \rz{77.47} & 60.37         & 72.73        & \rz{34.21} & \rz{47.70}  & \rz{49.16} & 36.05         & 40.61        & \rz{23.42} & \rz{38.37}  & \rz{52.19} & 25.39        & 35.48        \\ \hline
\rz{LISA$^\dagger$}                                & \rz{62.48} & \rz{86.37}  & \rz{95.75} & \rz{82.14}         & \rz{87.38}        & \rz{38.62} & \rz{49.42}  & \rz{75.82} & \rz{41.98}         & \rz{52.05}        & \rz{27.88} & \rz{46.86}  & \rz{68.23} & \rz{31.02}        & \rz{41.88}        \\
\rz{PixelLM$^\dagger$}                          & \rz{66.93} & \rz{85.71}  & \rz{93.28} & \rz{78.05}         & \rz{86.97}        & \rz{40.23} & \rz{52.25}  & \rz{77.28} & \rz{42.34}         & \rz{52.17}        & \rz{29.26} & \rz{47.42}  & \rz{55.83} & \rz{30.12}        & \rz{41.22}        \\ \hline
\rz{VG}        & \rz{33.56} & \rz{66.30}  & \rz{71.96} & \rz{51.40}         & \rz{63.15}        & \rz{30.42} & \rz{52.69}  & \rz{62.95} & \rz{33.08}         & \rz{43.05}        & \rz{22.70} & \rz{56.47}  & \rz{75.19} & \rz{26.35}        & \rz{46.72}        \\ 
\rz{VG+SAM}                 & \rz{40.37} & \rz{79.21}  & \rz{74.38} & \rz{60.58}         & \rz{69.58}        & \rz{37.22} & \rz{57.70}  & \rz{40.15} & \rz{39.36}         & \rz{37.98}        & \rz{25.83} & \rz{57.87}  & \rz{43.70} & \rz{29.36}        & \rz{39.07}        \\
\rz{VG+SAM2}              & \rz{34.30} & \rz{73.36}  & \rz{62.62} & \rz{54.15}         & \rz{62.10}        & \rz{31.69} & \rz{55.04}  & \rz{47.91} & \rz{34.27}         & \rz{37.14}        & \rz{21.11} & \rz{53.18}  & \rz{38.60} & \rz{24.40}        & \rz{33.27}      \\ 

\textbf{GeoPix} & \rz{\textbf{75.49}} & \rz{\textbf{92.37}}  & \rz{\textbf{96.27}} & \textbf{84.25}         & \textbf{89.82}        & \rz{50.73} & \rz{71.76}  & \rz{\textbf{80.63}} & 53.54         & \textbf{57.25}        & \rz{32.43} & \rz{\textbf{58.01}}  & \rz{59.88} & 35.37        & \textbf{45.24}        \\ \hline
\end{tabular}
}
\end{table}

==> tables/alb_fusion.tex <==
\begin{table}[]
\centering
\caption{Comparison of different fusion way of memory.}
\label{table:memory_fusion}
\begin{tabular}{l|c|cc}
\hline
\multirow{2}{*}{Memory Fusion} &  \multirow{2}{*}{Param.}  & \multicolumn{2}{c}{SIOR} \\ \cline{3-4} 
    &     &  mIoU   & cIoU      \\ \hline
argmax   &  0  &  76.24  & 85.21     \\
Conv2D   &  2.7K    &  80.42  & 88.82     \\
Conv3D   &  2.7K    &  \textbf{81.93}  & 89.64      \\ 
Attention       &  532.8K  &  79.90  & 88.31     \\
Dual Attention       &  34.6M   &  81.41  & \textbf{89.89}      \\ \hline

\end{tabular}
\end{table}

==> tables/ref_seg.tex <==
\begin{table*}[t]
\centering
\caption{\rz{Comparison of segmentation performance between using visual grounding-based bounding boxes as conditions with SAM/SAM2 and direct segmentation. All scores are evaluated and reported as percentages \hy{(combine with table 3)}}}
\label{table:ref_seg}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccccc|ccccc|ccccc}
\hline
\multirow{3}{*}{Method} & \multicolumn{5}{c|}{SIOR-T}                           & \multicolumn{5}{c|}{FAST-T}                           & \multicolumn{5}{c}{SOTA-T}                           \\ \cline{2-16} 
                        & Small & Medium & Large & \multicolumn{2}{c|}{Overall} & Small & Medium & Large & \multicolumn{2}{c|}{Overall} & Small & Medium & Large & \multicolumn{2}{c}{Overall} \\
                        & mIoU  & mIoU   & mIoU  & mIoU          & cIoU         & mIoU  & mIoU   & mIoU  & mIoU          & cIoU         & mIoU  & mIoU   & mIoU  & mIoU         & cIoU         \\ \hline
Visual Grounding        & 33.56 & 66.30  & 71.96 & 51.40         & 63.15        & 30.42 & 52.69  & 62.95 & 33.08         & 43.05        & 22.70 & 56.47  & 75.19 & 26.35        & 46.72        \\ 
Seg. with SAM                  & 40.37 & 79.21  & 74.38 & 60.58         & 69.58        & 37.22 & 57.70  & 40.15 & 39.36         & 37.98        & 25.83 & 57.87  & 43.70 & 29.36        & 39.07        \\
Seg. with SAM2                 & 34.30 & 73.36  & 62.62 & 54.15         & 62.10        & 31.69 & 55.04  & 47.91 & 34.27         & 37.14        & 21.11 & 53.18  & 38.60 & 24.40        & 33.27        \\ \hline
\textbf{End-to-end Seg.}                              & \textbf{75.49} & \textbf{92.37}  & \textbf{96.27} & \textbf{84.25}         & \textbf{89.82}        & \textbf{50.73} & \textbf{71.76}  & \textbf{80.63} & \textbf{53.54}         & \textbf{57.25}        & \textbf{32.43} & \textbf{58.01}  & \textbf{59.88} & \textbf{35.37}        & \textbf{45.24}        \\ \hline
\end{tabular}
}
\end{table*}

==> tables/seg.tex <==
\begin{table}[t]
\centering
\caption{Comparison of model performance on the multi-referring segmentation in the GeoPixInstruct}
\label{table:seg}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|cc|cc|cc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Dialogue} & \multicolumn{2}{c|}{SIOR-T} & \multicolumn{2}{c|}{FAST-T} & \multicolumn{2}{c}{SOTA-T} \\ \cline{3-8} 
   & & mIoU   & cIoU   & mIoU   & cIoU   & mIoU   & cIoU  \\ \hline
RRSIS & \ding{55} & 57.80  & 72.85 & 49.46  & 57.14 & 24.30  & 42.89  \\
RMSIN & \ding{55} & 65.10  & 78.27  & \textbf{56.59} & 56.88  & \textbf{44.42}  & 45.12  \\ \hline
LISA   & \ding{51} & 82.14  & 87.38  & 41.98  & 52.05  & 31.02  & 41.88  \\
PixelLM  & \ding{51} & 78.05  & 86.97  & 42.34  & 52.17  & 30.12  & 41.22  \\ \hline
\textbf{GeoPix}   & \ding{51} & \textbf{84.25}  & \textbf{89.82}  & 53.54  & \textbf{57.2}5  & 35.37  & \textbf{45.24}  \\ \hline
\end{tabular}
}
\end{table}
